Sequential Discontinuities of Feynman Integrals and the Monodromy Group

We generalize the relation between discontinuities of scattering amplitudes and cut diagrams to cover sequential discontinuities (discontinuities of discontinuities) in arbitrary momentum channels. The new relations are derived using time-ordered perturbation theory, and hold at phase-space points where all cut momentum channels are simultaneously accessible. As part of this analysis, we explain how to compute sequential discontinuities as monodromies and explore the use of the monodromy group in characterizing the analytic properties of Feynman integrals. We carry out a number of cross-checks of our new formulas in polylogarithmic examples, in some cases to all loop orders.

==> 3dstfigurev1.tex <==
 
\begin{figure}[t]
    \centering
\begin{tikzpicture}[baseline=-3.5]
\node at (0,0) {    \includegraphics[width=8cm]{diagrams/sstSurface.pdf}
    \includegraphics[width=8cm]{diagrams/ttsSurface.pdf}
    };
    \node[left,scale=0.8] at (-1,0.2) {$R^s$};
    \node[left,scale=0.8] at (-6,0.2) {$R^t$};
    \node[left,scale=0.8] at (-3,0.5) {$R^{st}$};
    \node[left,scale=0.5] at (-2,-0.5) {${\green{\circled{A}}}$}; 
    \node[left,scale=0.5] at (-3,-0.4) {${\circled{B}}$}; 
    \node[left,scale=0.5] at (-5.3,-0.1) {${\blue{\circled{C}}}$}; 
    \node[left] at (7,0.7) {$R^s$};
    \end{tikzpicture}
    \caption{The Landau surface for $\cM = \ln(-s)\ln(-t)$ is the hypersurface $\re s >0, \im s=0$ or $\re t>0, \im t=0$.
     Two 3D slicings of this surface are shown, with the shaded regions indicating that there {\it can} be a singularity for some value of the parameter not shown. The green path ${green{A}}$ computes $[\disc  \cM]_{R^s}$. 
     The black path $B$ computes $[\disc \cM]_{R^{st}}$. The blue path ${\blue{C}}$ computes $[\disc_s\cM]_{R^{st}}$ for which $\im t$ is not changed so the singularity in $R^t$ is avoided. 
    }
    \label{fig:stsurf}
\end{figure}

==> diagrams/tri2loopmassless3.tex <==
    \fmfstraight
	\fmfleft{L1}
	\fmfright{R1,R2}
	\fmf{plain_arrow,label=$p_3$}{L1,v1}
	\fmf{plain,label=$1$,tension=0.5,l.s=right}{v1,v2}
	\fmf{plain,label=$3$,l.s=right,tension=0}{v2,v3}
	\fmf{plain,label=$2$,l.s=right,tension=0.5}{v3,v1}
	\fmf{plain,label=$4$,tension=0.5}{v2,v4}
	\fmf{plain,label=$6$,tension=0.5}{v4,v5}
	\fmf{plain,label=$5$,tension=0.5,l.s=right}{v5,v3}
	\fmf{plain_arrow,tension=1.3}{R1,v4}
	\fmf{plain_arrow,tension=1.3}{R2,v5}
	\fmfv{label=$p_1$}{R2}	
	\fmfv{label=$p_2$}{R1}
